To Distill or Not to Distill? On the Robustness of Robust Knowledge Distillation

Arabic is known to present unique challenges for Automatic Speech Recognition (ASR). On one hand, its rich linguistic diversity and wide range of dialects complicate the development of robust, inclusive models. On the other, current multilingual ASR models are compute-intensive and lack proper comprehensive evaluations. In light of these challenges, we distill knowledge from large teacher models into smaller student variants that are more efficient. We also introduce a novel human-annotated dataset covering five under-represented Arabic dialects for evaluation. We further evaluate both our models and existing SoTA multilingual models on both standard available benchmarks and our new dialectal data. Our best-distilled model's overall performance ($45.0$\% WER) surpasses that of a SoTA model twice its size (SeamlessM4T-large-v2, WER=$47.0$\%) and its teacher model (Whisper-large-v2, WER=$55.1$\%), and its average performance on our new dialectal data ($56.9$\% WER) outperforms all other models. To gain more insight into the poor performance of these models on dialectal data, we conduct an error analysis and report the main types of errors the different models tend to make. The GitHub repository for the project is available at \url{https://github.com/UBC-NLP/distill-whisper-ar}.

==> sections/figures/training.tex <==
\begin{figure*}
  \centering

  \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{sections/assets/distillation-loss-kl.pdf}
    \caption{KL Divergence Loss}
    \label{fig:subfig1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{sections/assets/distillation-loss-ce.pdf}
    \caption{CE Loss}
    \label{fig:subfig2}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{sections/assets/distillation-loss-combined.pdf}
    \caption{Combined Loss}
    \label{fig:subfig3}
  \end{subfigure}

  \caption{Training loss for our distilled models.}
  \label{fig:overall}
\end{figure*}


==> sections/tables/co2-emission.tex <==
\begin{table*}[ht]
\begin{tabular}{ccccc}
\multicolumn{1}{c}{Experiment} & \multicolumn{1}{l}{Model} & \multicolumn{1}{l}{GPU Config} & \multicolumn{1}{l}{GPU Hours} & \multicolumn{1}{l}{Estimated CO2(kg CO2 equivalent)} \\
Evaluation                     & NA                        & 8xA100 + 4xA100(40G)           & 384                           & 66.36                                                \\
Distillation                   & distil-whisper-8-8        & 8xA100                         & 32                            & 5.53                                                 \\
Distillation                   & distil-whisper-16-16      & 8xA100                         & 48                            & 8.29                                                 \\
Distillation                   & distil-whisper-32-16      & 8xA100                         & 64                            & 11.06                                                \\
Distillation                   & distil-whisper-16-32      & 8xA100                         & 64                            & 11.06                                                \\
Distillation                   & distil-whisper-16-16++    & 8xA100                         & 96                            & 17.28                                                \\
Distillation                   & distil-whisper-32-16++    & 8xA100                         & 80                            & 13.82                                                \\
Finetuning and Misc.           & NA                        & 8x100                          & 160                           & 27.65                                                \\
Failed Runs                    & NA                        & 8xA100                         & 160                           & 27.65                                                \\
Total                          & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}           & 1088                          & 188.7                                               
\end{tabular}
\end{table*}

==> sections/tables/dummy-table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lll}
\toprule
Model & Data & Values \\
\midrule
0.0   & 0.0  & 0.0    \\
0.0   & 0.0  & 0.0  \\
\bottomrule
\end{tabular}
\caption{\label{tab:dummy-table}
This is a dummy table.
}
\end{table}

\begin{table*}[]
\centering
\begin{tabular}{lll}
\toprule
Model & Data & Values \\
\midrule
0.0   & 0.0  & 0.0    \\
0.0   & 0.0  & 0.0  \\
\bottomrule
\end{tabular}
\caption{\label{tab:dummy-table}
This is a dummy table in two columns.
}
\end{table*}

==> sections/tables/lambda-experiments.tex <==
\begin{table}[]
\centering
\begin{tabular}{c{1.5cm}ccc}
\toprule
Model    & $\lambda$ (\% F) & \begin{tabular}[c]{@{}c@{}}Avg.\\ Bench\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ IH\end{tabular} \\ \midrule

    
 \multirow{5}{*}{\centering\rotatebox{90}{DW-16-16}} & 10 (82.8) & 51.4/24.2 & 77.2/35.6 \\
 & 20 (74.7) &  42.2/19.6 & 69.1/29.1  \\ 
 & 40 (54.5) &  43.4/20.7 & 71.4/33.2  \\
 & 80 (28.0) &  40.0/18.6 & 66.3/27.8 \\
 & NA (0.0)  &  43.1/22.7 & 71.2/34.4 \\ \midrule

\multirow{5}{*}{\centering\rotatebox{90}{DW-32-16}} & 10 (82.8) & 40.2/18.7 & 65.6/26.4 \\
 & 20 (74.7) & 35.3/16.1 & 60.7/23.1 \\
 & 40 (54.5) & 39.8/19.2 & 66.9/29.3 \\
 & 80 (28.0 & 35.3/16.3 & 61.1/23.7  \\
 & NA (0.0) & 40.1/22.5 & 65.8/38.9 \\ \midrule
W-M & - & 54.3/32.9 & 76.4/44.1 \\
W-L-v2  & - & 33.2/19.0 & 68.2/38.9 \\ \bottomrule
\end{tabular}
\caption{\label{tab:lambda-experiments}
Results for different threshold ($\lambda$) values along with \textit{Whisper-medium} and \textit{Whisper-large-v2}. The average of reported results on test split of benchmarks and in-house data.~\textcolor{red}{Full results must be added in the appendix. Check \textbf{$\lambda$-experiments} sheet.} \KK{will do} 
}
\end{table}

==> sections/tables/main-double-precision.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h!]
\centering
\Large 
\renewcommand{\arraystretch}{1.}   %to squeeze table content low value means squeeze more
\resizebox{1.\linewidth}{!}{% reduce the text size, lower means smaller text size
\begin{tabular}{lcccccccccccc}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{CV15.0} & \multirow{2}{*}{MGB2} & \multirow{2}{*}{MGB2} & \multirow{2}{*}{MGB5} & \multirow{2}{*}{Fleurs} & \multicolumn{5}{c}{In-house Data}                                      \\
                       &                         &                       &                       &                       &                         & ALG          & JOR         & PAL         & UAE          & YEM          \\ \midrule
Amazon              &                         &                       &                       &                       &                         &              &             &             &              &              \\ \midrule
XLS-R                  & 89.72/39.39             & 97.56/53.13           & 98.73/61.64           & 99.51/68              & 94.86/43.9              & 99.73/66.95  & 99.13/61.39 & 99.14/61.06 & 99.39/64.56  & 99.52/63.64  \\
HuBERT                 & 55.17/18.9              & 49.59/17.34           & 25.23/9.54            & 92.36/45.52           & 34.85/10.9              & 96.81/44.28  & 65.21/23.27 & 73.79/27.94 & 83.02/36.69  & 90.53/38.76  \\
W-FT                   & 35.84/21.89             & 15.29/8.13            & 48.92/26.85           & 101.35/62.3           & 9.81/3.44               & 115.5/69.63  & 67.82/37.19 & 69.62/35.41 & 105.92/69.11 & 107.14/64.82 \\ \midrule
W-S                    & -/-                     & 55.32/26.35           & 77.42/45.07           & 113.1/74.34           & 40.16/11.37             & -/-          & -/-         & -/-         & -/-          & -/-          \\
W-L                    &                         &                       &                       &                       &                         &              &             &             &              &              \\
W-L-V2                 & 19.34/6.67              & 34.74/17.75           & 43.53/21.87           & 82.97/49.12           & 11.56/3.74              & 103.44/81.94 & 72.8/58.95  & 51.92/19.42 & 102.83/83.48 & 102.66/81.26 \\
W-L-v3                 & 15.75/5.16              & 15.91/7.64            & 35.68/17.34           & 79.83/44.57           & 9.71/3.19               & 101.89/65.4  & 43.55/16.27 & 53.4/22.73  & 63.35/32.68  & 76.14/38.91  \\
SM4T-M                 & 16.26/5.66              & 19.49/8.96            & 41.41/21.66           & 83.77/46.58           & 8.68/3.64               & 81.05/39.69  & 46.33/15.86 & 55.19/20.11 & 59.84/24.65  & 68.93/29.5   \\
SM4T-L                 & 19.79/7.34              & 21.79/10.54           & 44.37/22.58           & 89.85/52.05           & 11.12/5.14              & 92.14/51.95  & 41.52/14.61 & 49.46/17.15 & 55.88/23.33  & 69.73/30.71  \\
SM4T-L                 & 11.26/3.52              & 17.33/8.73            & 36.2/18.55            & 89.11/53.73           & 7.64/3.98               & 92.14/51.95  & 41.52/14.61 & 49.46/17.15 & 55.88/23.33  & 69.73/30.71  \\ \midrule
D-W-8-8                & 89.72/39.39             & 97.56/53.13           & 98.73/61.64           & 99.51/68              & 94.86/43.9              & 99.73/66.95  & 99.13/61.39 & 99.14/61.06 & 99.39/64.56  & 99.52/63.64  \\
D-W-16-16              & 89.72/39.39             & 97.56/53.13           & 98.73/61.64           & 99.51/68              & 94.86/43.9              & 99.73/66.95  & 99.13/61.39 & 99.14/61.06 & 99.39/64.56  & 99.52/63.64  \\
D-W-32-16              & 89.72/39.39             & 97.56/53.13           & 98.73/61.64           & 99.51/68              & 94.86/43.9              & 99.73/66.95  & 99.13/61.39 & 99.14/61.06 & 99.39/64.56  & 99.52/63.64  \\
D-W-16-32              & 89.72/39.39             & 97.56/53.13           & 98.73/61.64           & 99.51/68              & 94.86/43.9              & 99.73/66.95  & 99.13/61.39 & 99.14/61.06 & 99.39/64.56  & 99.52/63.64 \\ \bottomrule 
\end{tabular}
}
\caption{ \label{main-results}
Main Results. \textcolor{red}{Abdul2Himself: All results are dummy values to get the structure of the table. Fill and verify the values.}
}
\end{table*}



==> sections/tables/not-main.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h!]
\centering
\Large 
\renewcommand{\arraystretch}{1.}   %to squeeze table content low value means squeeze more
\resizebox{1.\linewidth}{!}{% reduce the text size, lower means smaller text size
\begin{tabular}{lcccccccccccccc}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Size}  & \multirow{2}{*}{CV15.0} & \multirow{2}{*}{MGB2} & \multirow{2}{*}{MGB3} & \multirow{2}{*}{MGB5} & \multirow{2}{*}{Fleurs} & \multicolumn{5}{c}{In-house Data} & \multirow{2}{*}{Avg.}                                     \\
                       &               &          &                       &                       &                       &                         & ALG          & JOR         & PAL         & UAE          & YEM          \\ \midrule
Amazon & -/- & -/- & -/- & -/- & -/- & -/- & 83.6/70.2 & 45.5/25.6 & 52.4/29.0 & 58.8/40.8 & 64.7/43.5 & 61.0/41.8 \\ \midrule

XLS-R & 0.96 & 89.7/39.4 & 97.6/53.1 & 98.7/61.6 & 99.5/68.0 & 94.9/43.9 & 99.7/67.0 & 99.1/61.4 & 99.1/61.1 & 99.4/64.6 & 99.5/63.6 & 97.7/58.4 \\

HuBERT & 0.31 & 55.2/18.9 & 49.6/17.3 & \textbf{25.2/9.5} & 92.4/45.5 & 34.9/10.9 & 96.8/44.3 & 65.2/23.3 & 73.8/27.9 & 83.0/36.7 & 90.5/38.8 & 66.7/27.3 \\

W-FT & 1.5 & 35.8/21.9 & \textbf{15.3/8.1} & 48.9/26.9 & 101.4/62.3 & 9.8/3.4 & 115.5/69.6 & 67.8/37.2 & 69.6/35.4 & 105.9/69.1 & 107.1/64.8 & 67.7/39.9\\ \midrule

MMS-all & 1.0 & 106.4/80.9 & 39.3/13.4 & 75.3/34.6 & 89.7/45.9 & 23.8/6.3 & 100.2/78.0 & 89.8/55.4 & 99.9/75.1 & 100.1/78.1 & 100.2/76.6 & 82.5/54.4 \\ \hdashline

SM4T-M & 1.2 & 16.3/5.7 & 19.5/9.0 & 41.4/21.7 & 83.8/46.6 & 8.7/3.6 & 81.1/39.7 & 46.3/15.9 & 55.2/20.1 & 59.8/24.7 & 68.9/29.5 & 48.1/21.7 \\

SM4T-L-v1 & 2.3 & 19.8/7.3 & 21.8/10.5 & 44.4/22.6 & 89.9/52.1 &  11.1/5.1 & 87.9/47.8 & 50.7/18.8 & 57.5/23.1 &  61.8/27.4 & 72.2/32.5 & 51.7/24.7 \\

SM4T-L-v2 & 2.3 & \textbf{11.3/3.5} & 17.3/8.7 & 36.2/18.6 & 89.1/53.7 & \textbf{7.6/4.0} & 92.1/52.0 & \textbf{41.5/14.6} & \textbf{49.5/17.2} & \textbf{55.9/23.3} & 69.7/30.7 & \textbf{47.0/22.6} \\ \hdashline 

W-S & 0.24 & 40.3/16.4 & 46.8/24.7 & 81.4/51.9 & 226.5/164.8 & 28.2/8.7 & 130.71/84.67 & 68.6/32.93 & 73.84/36.25 & 97.81/59.68 & 107.1/66.7 & 80.8/45.7 \\

W-M & 0.77 & 29.8/13.2 & 33.1/18.5 & 64.3/39.5 & 127.7/88.3 & 16.4/5.1 & 103.7/69.9 & 50.5/21.1 & 58.7/24.7 & 82.5/52.6 & 86.8/52.0 &  65.4/38.5\\

W-L-v2 & 1.5 & 19.6/7.8 & 26.5/15.3 & 53.0/33.0 & 99.2/68.9 & 11.4/3.6 & 106.4/71.7 & 42.3/17.0 & 51.1/22.3 & 63.8/38.2 & 77.3/45.5 & 55.1/32.3 \\

W-L-v3 & 1.5 & 15.8/5.2 & 15.9/7.6 & 35.7/17.3 & 79.8/44.6 & 9.7/3.2 & 101.9/65.4 & 43.6/16.3 & 53.4/22.7 & 63.4/32.7 & 76.1/38.9 & 49.5/25.4 \\ \midrule

D-W-8-8 & 0.44 & 32.7/12.3 & 39.6/17.8 & 64.9/36.6 & 89.7/53.0 & 29.8/11.4 & 91.4/48.2 & 66.2/29.0 & 73.2/33.0 & 78.0/38.4 & 82.9/41.5 & 64.8/32.1\\

D-W-16-16 & 0.80 & 22.1/7.2 & 26.0/10.8 & 50.5/25.1 & 82.4/43.3 & 18.8/6.6 & 83.0/38.5 & 50.4/18.2 & 61.0/23.3 & 64.6/27.7 & 72.7/31.6 & 53.2/23.2 \\

D-W-32-16 & 1.12 & 18.8/5.9 & 21.1/8.9 & 43.8/21.4 & \textbf{78.9/40.4} & 14.2/4.8 & \textbf{79.5/33.4} & 44.4/14.7 & 55.0/19.5 & 58.1/22.8 & \textbf{68.5/28.1} & 48.2/20.0 \\

D-W-16-32 & 1.22 & 21.5/7.3 & 25.0/10.7 & 49.1/26.3 & 83.0/47.5 & 18.4/6.0 & 84.3/44.0 & 49.8/18.0 & 60.3/25.4 & 64.4/29.0 & 73.8/36.8 & 53.0/25.1\\ 

\hdashline
D-W-16-16++ & 0.80 & 20.0/6.6 & 23.6/10.1 & 47.7/23.5 & 85.2/44.7 & 15.2/5.1 & 84.1/37.9 & 46.4/16.2 & 56.8/20.9 & 61.2/24.9 & 73.9/32.7 & 51.4/22.3 \\
D-W-32-16++ & 1.12 & 18.2/5.7 & 21.3/9.3 & 44.2/22.1 & 89.7/49.0 & 13.5/4.5 & 80.0/35.9 & 43.6/14.5 & 54.3/18.9 & 57.3/23.1 & 71.7/30.1 & 49.4/21.3 \\

\bottomrule 
\end{tabular}
}
\caption{ \label{main-results}
WER/CER scores after normalization and removing diacritics. Average is the mean score across all the evaluation sets. We report on test split of each datasets.
Abbreviations. W - Whisper, FT - Finetuned, M - Medium, L - Large, S - Small, D - Distil.
}
\end{table*}

==> sections/tables/raw-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h!]
\centering
\Large 
\renewcommand{\arraystretch}{1.}   %to squeeze table content low value means squeeze more
\resizebox{1.\linewidth}{!}{% reduce the text size, lower means smaller text size
\begin{tabular}{lccccccccccccc}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Size} & \multirow{2}{*}{CV15.0} & \multirow{2}{*}{MGB2} & \multirow{2}{*}{MGB3} & \multirow{2}{*}{MGB5} & \multirow{2}{*}{Fleurs} & \multicolumn{5}{c}{In-house Data} & \multirow{2}{*}{Avg.} \\ & & &  & & & & ALG & JOR & PAL & UAE & YEM \\ 
\midrule
Amazon & -/- & -/- & -/- & -/- & -/- & -/- & 88.0/71.6 & 59.2/29.1 & 63.4/32.2 & 71.1/44.3 & 77.4/47.7 & 71.8/45.0 \\ 
\midrule

XLS-R & 0.96 & 92.7/46.7 & 97.7/54.5 & 99.1/64.5 & 99.6/70.1 & 95.1/45.4 & 99.7/68.0 & 99.3/62.9 & 99.2/62.8 & 99.5/66.4 & 99.7/66.4 & 98.2/60.8 \\

HuBERT &0.31 & 76.5/31.0 & 59.4/20.3 & 43.3/16.5 & 95.0/48.7 & 48.9/14.4 & 96.2/45.6 & 70.6/25.4 & 81.5/31.4 & 87.9/39.9 & 91.3/40.8 & 75.1/31.4 \\

W-FT & 1.5 & 70.0/33.8 & 29.4/10.9 & 60.1/32.2 & 105.0/64.3 & 28.7/7.3 & 114.5/70.3 & 75.1/39.0 & 81.3/38.7 & 113.7/70.9 & 110.1/65.6 & 78.8/43.3 \\ \midrule

MMS-all & 1.0 & 106.0/82.5 & 40.3/14.0 & 77.7/38.1 & 90.4/48.5 & 28.8/7.8 & 100.2/77.8 & 91.5/56.2 & 100.0/75.8 & 100.1/78.4 & 100.1/76.8 & 83.5/55.6 \\ \hdashline

SM4T-M & 1.2 & 42.3/18.2 & 28.1/11.2 & 50.2/26.8 & 88.2/50.8 & 19.5/6.0 & 84.5/42.8 & 55.2/18.7 & 63.0/23.0 & 68.0/28.1 & 79.4/34.5 & 57.8/26.0 \\

SM4T-L-v1 & 2.3 & 44.2/19.1 & 25.9/11.7 & 52.5/27.6 & 92.8/55.9 & 22.6/7.6 & 89.7/50.3 & 59.1/21.7 & 64.7/25.8 & 69.0/30.3 & 81.5/37.0 & 60.2/28.7 \\

SM4T-L-v2 & 2.3 & 37.7/15.8 & 22.4/9.9 & 46.7/23.9 & 92.1/58.4 & 19.8/6.5 & 94.8/55.2 & 51.3/17.6 & 58.5/20.1 & 65.6/26.9 & 80.6/35.5 & 57.0/27.0\\ \hdashline 

W-S & 0.24 & 68.9/31.8 & 49.5/25.7 & 84.8/55.4 & 228.6/164.5 & 33.4/10.3 & 129.15/87.85 & 75.25/36.55 & 79.73/39.3 & 103.83/63 & 112.69/70.69 & 96.6/58.5 \\ 

W-M & 0.77 & 55.1/24.2 & 37.6/19.6 & 71.5/43.7 & 129.7/89.4 & 24.0/7.1 & 103.9/71.4 & 59.0/23.9 & 66.8/27.6 & 90.7/55.7 & 95.2/56.2 & 73.4/41.9 \\

W-L-v2 & 1.5 & 46.9/19.6 & 33.7/16.9 & 60.6/37.7 & 101.1/71.1 & 19.7/5.6 & 106.9/74.6 & 51.2/19.6 & 60.2/25.2 & 73.2/41.2 & 86.9/50.1 & 67.4/38.3 \\

W-L-v3 & 1.5 & 43.2/16.9 & 20.4/8.6 & 44.6/22.5 & 82.0/47.7 & 16.4/4.8 & 103.8/68.9 & 52.7/18.9 & 64.3/26.4 & 72.3/35.9 & 86.0/43.3 & 58.6/29.4 \\ \midrule

D-W-8-8 & 0.44 & 55.0/23.2 & 44.4/19.2 & 69.2/40.4 & 91.0/55.5 & 36.1/13.3 & 91.5/49.6 & 71.4/31.2 & 78.4/35.6 & 82.5/41.2 & 87.5/44.9 & 70.7/35.4 \\

D-W-16-16 & 0.80 & 48.0/18.9 & 33.2/12.5 & 57.1/29.6 & 84.1/46.2 & 26.2/8.5 & 83.8/40.2 & 57.8/20.5 & 68.2/26.2 & 72.0/31.0 & 80.0/35.6 & 61.0/26.9 \\

D-W-32-16 & 1.12 & 45.6/17.7 & 27.7/10.3 & 51.2/26.1 & 80.9/43.4 & 22.0/6.6 & 80.5/35.1 & 52.6/17.1 & 62.9/22.4 & 66.7/26.3 & 77.3/32.6 & 56.7/23.8 \\

D-W-16-32 & 1.22 & 47.4/18.8 & 29.9/11.8 & 55.5/30.7 & 84.7/50.2 & 26.0/7.9 & 84.8/45.7 & 57.4/20.4 & 67.4/28.2 & 71.7/32.3 & 81.5/40.9 & 60.6/28.7 \\
\hdashline
D-W-16-16++ & 0.80 & 46.3/18.2 & 30.7/11.7 & 54.8/28.1 & 87.4/47.4 & 22.0/6.8 & 84.6/39.6 & 54.1/18.5 & 64.7/23.9 & 69.6/28.4 & 81.4/36.7 & 59.6/25.9 \\
D-W-32-16++ & 1.12 & 45.1/17.4 & 28.4/10.8 & 51.3/26.8 & 91.6/51.6 & 21.1/6.3 & 80.9/37.7 & 51.9/17.0 & 62.3/21.8 & 66.1/26.6 & 80.2/34.5 & 57.9/25.1 \\

\bottomrule 
\end{tabular}
}
\caption{ \label{raw-results}
WER/CER scores on orthographic transcription produced by the models. Average is the mean score across all the evaluation sets. We report on the test split of each dataset. Abbreviations. W - Whisper, FT - Finetuned, M - Medium, L - Large, S - Small, D - Distil. \textcolor{red}{Tables 3 and 4 can be merged.}
}

\end{table*}


